Power in the Pipeline

This paper provides the first comprehensive empirical analysis of the role of natural gas for the domestic and international distribution of power. The crucial role of pipelines for the trade of natural gas determines a set of network effects that are absent for other natural resources such as oil and minerals. Gas rents are not limited to producers but also accrue to key players occupying central nodes in the gas network. Drawing on our new gas pipeline data, this paper shows that gas betweenness-centrality of a country increases substantially the ruler's grip on power as measured by leader turnover. A main mechanism at work is the reluctance of connected gas trade partners to impose sanctions, meaning that bad behavior of gas-central leaders is tolerated for longer before being sanctioned. Overall, this reinforces the notion that fossil fuels are not just poison for the environment but also for political pluralism and healthy regime turnover.

==> table/reg_durability.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Leader durability}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Cheibub}&\multicolumn{1}{c}{Archigos}\\
\hline
L.Ln(BC)            &    -0.05\sym{***}&    -0.06\sym{**} \\
                    &   [0.02]         &   [0.02]         \\
[1em]
L.DC                &     0.04         &     0.02         \\
                    &   [0.04]         &   [0.06]         \\
[1em]
lnpop               &     0.00         &    -0.03         \\
                    &   [0.16]         &   [0.28]         \\
[1em]
ln(GDP)             &     0.06         &     0.19         \\
                    &   [0.09]         &   [0.17]         \\
[1em]
Log(Oil rents (\% of&     0.00         &    -0.00         \\
GDP))               &   [0.00]         &   [0.00]         \\
[1em]
Log(Natural gas     &     0.00\sym{*}  &     0.00\sym{**} \\
rents (\% of GDP))  &   [0.00]         &   [0.00]         \\
\hline
\(R^{2}\)           &    0.210         &    0.224         \\
Mean dep var        &     0.20         &     0.17         \\
FE year             &      Yes         &      Yes         \\
FE ctry             &      Yes         &      Yes         \\
Observations        &     1862         &     1260         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Error clustered at the country level.}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> table/reg_growth.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Democracy, Growth, and quality of the government}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{PolityIV}&\multicolumn{1}{c}{V-dem}&\multicolumn{1}{c}{FH}&\multicolumn{1}{c}{ln(GDP)}&\multicolumn{1}{c}{QoG}&\multicolumn{1}{c}{St.Cap.}\\
\hline
L.Ln(BC)            &    -0.20         &    -0.01         &    -0.09         &     0.01         &     0.00         &    -0.00         \\
                    &   [0.46]         &   [0.33]         &   [0.40]         &   [0.36]         &   [0.25]         &   [0.93]         \\
[1em]
L.DC                &    -0.20         &    -0.01         &     0.02         &    -0.01         &    -0.01\sym{**} &     0.02         \\
                    &   [0.62]         &   [0.68]         &   [0.91]         &   [0.54]         &   [0.03]         &   [0.54]         \\
[1em]
lnpop               &     0.78         &     0.01         &     0.10         &    -0.47\sym{***}&     0.08\sym{***}&    -0.05         \\
                    &   [0.40]         &   [0.73]         &   [0.78]         &   [0.00]         &   [0.00]         &   [0.68]         \\
[1em]
Log(Oil rents (\% of&    -0.02\sym{*}  &    -0.00         &    -0.01         &     0.01\sym{**} &     0.00         &     0.00         \\
GDP))               &   [0.08]         &   [0.42]         &   [0.24]         &   [0.04]         &   [0.77]         &   [0.33]         \\
[1em]
Log(Natural gas     &    -0.01         &    -0.00         &    -0.00         &    -0.00\sym{*}  &    -0.00         &    -0.00         \\
rents (\% of GDP))  &   [0.41]         &   [0.46]         &   [0.59]         &   [0.09]         &   [0.14]         &   [0.91]         \\
\hline
\(R^{2}\)           &    0.891         &    0.938         &    0.924         &    0.983         &    0.954         &    0.960         \\
Mean dep var        &     2.92         &     0.40         &     5.91         &     9.11         &     0.57         &     0.50         \\
FE year             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
FE ctry             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Observations        &     2989         &     3190         &     3030         &     3173         &     2467         &     2675         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Error clustered at the country level.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> table/reg_growth_2.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Democracy, Growth, and quality of the government}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{PolityIV}&\multicolumn{1}{c}{V-dem}&\multicolumn{1}{c}{FH}&\multicolumn{1}{c}{ln(GDP)}&\multicolumn{1}{c}{QoG}&\multicolumn{1}{c}{St.Cap.}\\
\hline
L.Ln(BC)            &    -0.20         &    -0.01         &    -0.09         &     0.01         &     0.00         &    -0.00         \\
                    &   [0.46]         &   [0.33]         &   [0.40]         &   [0.36]         &   [0.25]         &   [0.93]         \\
[1em]
L.DC                &    -0.20         &    -0.01         &     0.02         &    -0.01         &    -0.01\sym{**} &     0.02         \\
                    &   [0.62]         &   [0.68]         &   [0.91]         &   [0.54]         &   [0.03]         &   [0.54]         \\
[1em]
lnpop               &     0.78         &     0.01         &     0.10         &    -0.47\sym{***}&     0.08\sym{***}&    -0.05         \\
                    &   [0.40]         &   [0.73]         &   [0.78]         &   [0.00]         &   [0.00]         &   [0.68]         \\
[1em]
Log(Oil rents (\% of&    -0.02\sym{*}  &    -0.00         &    -0.01         &     0.01\sym{**} &     0.00         &     0.00         \\
GDP))               &   [0.08]         &   [0.42]         &   [0.24]         &   [0.04]         &   [0.77]         &   [0.33]         \\
[1em]
Log(Natural gas     &    -0.01         &    -0.00         &    -0.00         &    -0.00\sym{*}  &    -0.00         &    -0.00         \\
rents (\% of GDP))  &   [0.41]         &   [0.46]         &   [0.59]         &   [0.09]         &   [0.14]         &   [0.91]         \\
\hline
\(R^{2}\)           &    0.891         &    0.938         &    0.924         &    0.983         &    0.954         &    0.960         \\
Mean dep var        &     2.92         &     0.40         &     5.91         &     9.11         &     0.57         &     0.50         \\
FE year             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
FE ctry             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Observations        &     2989         &     3190         &     3030         &     3173         &     2467         &     2675         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Error clustered at the country level.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}


==> table/reg_sanction.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Sanctions (sample restricted)}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &Any Sanction         &                  &Arms Sanctions         &                  &Sanctions to prevent war         &                  \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Network}&\multicolumn{1}{c}{Others}&\multicolumn{1}{c}{Network}&\multicolumn{1}{c}{Others}&\multicolumn{1}{c}{Network}&\multicolumn{1}{c}{Others}\\
\hline
L.Ln(BC)            &    -0.03         &     0.02         &    -0.04\sym{**} &     0.01         &    -0.03\sym{**} &     0.01         \\
                    &   [0.02]         &   [0.02]         &   [0.02]         &   [0.02]         &   [0.01]         &   [0.01]         \\
[1em]
L.DC                &     0.09\sym{**} &    -0.10\sym{***}&     0.10\sym{***}&    -0.05         &     0.07\sym{**} &    -0.06\sym{**} \\
                    &   [0.03]         &   [0.04]         &   [0.03]         &   [0.04]         &   [0.03]         &   [0.02]         \\
[1em]
lnpop               &     0.08         &    -0.12         &     0.10         &    -0.06         &     0.10\sym{*}  &    -0.08         \\
                    &   [0.08]         &   [0.12]         &   [0.07]         &   [0.09]         &   [0.05]         &   [0.06]         \\
[1em]
ln(GDP)             &    -0.01         &    -0.09         &    -0.03         &    -0.14\sym{*}  &    -0.01         &    -0.03         \\
                    &   [0.05]         &   [0.11]         &   [0.04]         &   [0.07]         &   [0.02]         &   [0.04]         \\
[1em]
Log(Oil rents (\% of&    -0.00         &    -0.00         &    -0.00         &    -0.00         &    -0.00         &    -0.00\sym{**} \\
GDP))               &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         \\
[1em]
Log(Natural gas     &     0.00         &    -0.01\sym{**} &     0.00         &    -0.00         &    -0.00         &    -0.00\sym{***}\\
rents (\% of GDP))  &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         &   [0.00]         \\
\hline
\(R^{2}\)           &    0.543         &    0.580         &    0.582         &    0.599         &    0.526         &    0.623         \\
Mean dep var        &    0.088         &    0.411         &    0.054         &    0.138         &    0.028         &    0.112         \\
FE year             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
FE ctry             &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Observations        &     3173         &     3173         &     3173         &     3173         &     3173         &     3173         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Error clustered at the country level.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{table}

